Do Language Models Exhibit Human-like Structural Priming Effects?

We explore which linguistic factors -- at the sentence and token level -- play an important role in influencing language model predictions, and investigate whether these are reflective of results found in humans and human corpora (Gries and Kootstra, 2017). We make use of the structural priming paradigm, where recent exposure to a structure facilitates processing of the same structure. We don't only investigate whether, but also where priming effects occur, and what factors predict them. We show that these effects can be explained via the inverse frequency effect, known in human priming, where rarer elements within a prime increase priming effects, as well as lexical dependence between prime and target. Our results provide an important piece in the puzzle of understanding how properties within their context affect structural prediction in language models.

==> sections/9_conclusion.tex <==
\section{Conclusions}
% are lms plausible cognitive models?
% can we investigate predictive processing and evidence of abstract structural representations in more depth (w-pe = necessary) 
Through our investigation of structural prediction in LMs, we contribute a \textit{token}-level priming metric to measure priming, conducting experiments which shed light on a) \textit{where} within a sentence structural priming in models takes place, as well as b) \textit{what} factors relating to lexico-semantic overlap, structural preference and predictability(of the primes and targets) predict priming effects in models. 
\new{We find model behaviour relatively consistent, with no clear pattern of difference between foundation vs. alignment tuned(?)}

Our results suggest that models' structural predictions are highly tied to these specific lexical items, and that their behaviour also incorporates systematic properties of human production preferences learnt from the training data.
These findings form an important piece in the puzzle of understanding how context affects structural predictions in language models.


% Investigating the extent to which language models are influenced by structure and semantics when making upcoming predictions, has the potential to help answer long standing debates within theoretical linguistics e.g.~\cite{linzen2021syntactic}, as well as shed light on the influence of contextual cues acting on model predictions which can have implications for emerging work within in-context learning and prompt engineering \citep{min-etal-2022-rethinking, han-etal-2023-understanding}.

% For our experiments we make use of the Prime-LM corpus of \citet{sinclair2022structural}, which provides a rich set of prime-target pairs under various conditions, such as the degree of semantic similarity and lexical overlap.
% We extend Prime-LM with more fine-grained conditions for lexical overlap and examine a suite of contemporary LLMs, seeking to explore how model scale and alignment affect priming effects. 
% One peculiarity of structural priming in LMs that we investigate is their \textit{asymmetric priming} behaviour, in which a model shows strong priming effects only in one structural direction.
% % While asymmetry in effect between structures is somewhat expected from a human perspective \citep{JAEGER201357,BERNOLET2014113}, 
% We show that by measuring priming effects at the \textit{token-level} we obtain a more nuanced insight that explains some of the asymmetry.
% This token-level analysis also demonstrates that priming manifests itself highly differently across different tokens in the target, and provides a detailed overview of the lexico-semantic interactions that are at play.
% Finally, we set up an elaborate regression experiment to uncover more precisely which linguistic factors are the driving forces for priming behaviour. 
% We demonstrate that priming in LMs is strongly driven by \textit{structural preference}, following a similar \textit{inverse frequency effect} that is prevalent in human priming \citep{grieswulff2005,Jaeger2008cog}.

% \jj{Wrapping up now: final little paragraph here should have a high-level reflection on the contribution of our work, and the broader line of work that it falls under. (thinking of piantadosi/lake+baroni/futrell/michael c frank etc.}
%


==> sections/_intro_notes.tex <==
% Story draft:
% - What is priming: can tell about abstract structure can also tell about what influences models to make predictions
% - prior work explored many factors broadly to inspect whether these effects exist for models
% we need to also understand these effects more deeply in terms of: 
% 0) consistency are they consistent across models? are they consistent across structures? 
% 1) at a more fine-grained level if we are to understand where these effects have the most likelihood of taking place (e.g. we measure in comprehension but e.g. to understand generation we need a per-token view)
% 2) how frequency effects play a role: this has not been focussed on in prior experiments: surprisal and structural preference 
% 3) can we begin to predict priming effects via these methods?  lexico-semantic simlarity, and surprisal are predictive of model expectations about strucutures, however this does not fully explain the effects we see (these are very complex and we know from human literature there are far more factors at play)  
% Why do we care? these results are interesting because it tells us something about the degree of abstract relationships these models encode from data, and develops our understanding of how context shapes predictions which can have implication for better design and evaluation of prompts/tasks/instructions(?) 
% This also has some angle of making use of models to *explore* corpus data and understand large scale human language patterns through this sort of method (too circular?)



% - Relationship between lex sem in a per-token manner
% - Novel: frequency and likelihood
% - Novel: relative contribution of factors in combination $\rightarrow$ how to predict priming

% Prior work focussed on the question of whether or not priming effects are present within models, and thus did not focus on the differences in PE observed across structures, nor seek to pinpoint where these effects take place within a target sentence. 
% Focussing in on this difference, we conduct a detailed and complementary analysis to X, tackling the unanswered question of the role of this cognitive bias in humans and how in fact these results indicate model sensitivity to the \textit{inverse frequency effect}, whereby humans are more likely to repeat, or be primed by rarer or more surprising language. 
% are the asymmetrical priming effects reported in X explained by a) human preference for PO rather than DO b) verb selectional preference for one or other structure c) surprisal for the sentence as a whole b) lexical frequency at the word level? 
% To answer these questions, we propose an updated measure of per-token PE, which allows for finer-grained observation of where priming effects take place, allowing us to test 

\begin{comment}

Humans and language models are influenced by many factors within their linguistic context when it comes to making predictions about upcoming words. 
There is much behavioural evidence of readers and listeners engaging in lexical, semantic and structural prediction \citep{trueswell1993verb,kuperberg2016we,shain2020fmri,tooley2023structural}. 
One paradigm designed to investigate the presence of abstract structural representations in humans is \textbf{structural priming}, which, if present, should also influence the processing of upcoming structures.

<cut stuff now below>

We turn our attention to the rich literature on factors that have been shown to impact priming in human language processing.
Contrary to earlier work, we focus in particular on analyses from corpus linguistics, that have shown priming to be prevalent not only in spoken dialogue, but written text as well \citep{gries_kootstra_2017}.
By focusing on factors derived from corpus linguistics, we can provide a better account for the priming behaviour of language models, as they must have acquired this based on corpus data patterns.

\end{comment}

Humans and language models are influenced by many factors within their linguistic context when it comes to making predictions about upcoming words. 
There is much behavioural evidence of readers and listeners engaging in lexical, semantic and structural prediction \citep{trueswell1993verb,kuperberg2016we,shain2020fmri,tooley2023structural}. 
One paradigm designed to investigate the presence of abstract structural representations in humans is \textbf{structural priming}, which, if present, should also influence the processing of upcoming structures.

<cut stuff now below>

We turn our attention to the rich literature on factors that have been shown to impact priming in human language processing.
Contrary to earlier work, we focus in particular on analyses from corpus linguistics, that have shown priming to be prevalent not only in spoken dialogue, but written text as well \citep{gries_kootstra_2017}.
By focusing on factors derived from corpus linguistics, we can provide a better account for the priming behaviour of language models, as they must have acquired this based on corpus data patterns.

Prior work found evidence of priming in models. However how this works precisely in the absence of lexical overlap remains unclear 
% However understanding \textit{where} these effects are observed within a target sentence, and predicting the strength of the priming effects remains less well understood.
%It remains puzzling, however, \textit{how} structural priming manifests in language models, and what factors drive this behaviour.


Prior work focused on the question of whether or not priming effects are present within models, and thus did not focus on the differences in PE observed across structures, nor seek to pinpoint where these effects take place within a target sentence. 
Focusing in on this difference, we conduct a detailed and complementary analysis to X, tackling the unanswered question of the role of this cognitive bias in humans and how in fact these results indicate model sensitivity to the \textit{inverse frequency effect}, whereby humans are more likely to repeat, or be primed by rarer or more surprising language. 
are the asymmetrical priming effects reported in X explained by a) human preference for PO rather than DO b) verb selectional preference for one or other structure c) surprisal for the sentence as a whole b) lexical frequency at the word level? 
To answer these questions, we propose an updated measure of per-token PE, which allows for finer-grained observation of where priming effects take place, allowing us to test 




%priming exists in humans and models. 


%priming is typically stronger in one or other structure: inverse frequency. prior work does not focus on this, however sinclair et al show the opposite
Priming effects in humans are typically stronger for the \textit{less} frequent structure: typically the \textsc{PO} in English corpora~\citep{bock2000persistence,reitter2011computational}.
This \textit{inverse frequency} effect extends to other properties of structures themselves, which we make one of our foci in this paper. 

% \textit{inverse frequency effect}, whereby humans are more likely to repeat, or be primed by, rarer and thus more surprising language.


%what do we do and why: we explore this difference in more detail, needing better measure and conditions to understand what predicts these effects.
Through our investigation of structural prediction in LMs, we contribute a \textit{token}-level priming metric to measure priming, conducting experiments which shed light on a) \textit{where} within a sentence structural priming in models takes place, as well as b) \textit{what} factors relating to lexico-semantic overlap, structural preference and predictability(of the primes and targets) predict priming effects in models. 
%
We find that models' structural predictions are highly tied to specific lexical items, as well as incorporating systematic properties of human production preferences learnt from the training data.
These findings form an important piece in the puzzle of understanding how context affects structural predictions in language models.


\as{
% "\new{Specifically, our token-level analysis demonstrates that priming manifests itself highly differently across different tokens in the target, depending on lexical overlap properties, and demonstrate that priming in LMs is strongly driven by \textit{structural preference}, following a similar \textit{inverse frequency effect} that is prevalent in human priming \citep{grieswulff2005,Jaeger2008cog}.}"

}



==> sections/notes.tex <==
\section{Notes}

For instance, Chang et al. (2003; see also Yi \& Koenig, 2016; Ziegler \& Snedeker, 2018) found that location-theme locative sentences (“The maid rubbed the table with polish”) led to a higher proportion of location–theme responses (“The farmer heaped the wagon with straw”) as compared to theme-location locatives (“The maid rubbed polish onto the table”). This occurred despite the two locative types having the same syntactic structure (both NP-V-NP-PP). Thus, priming is sensitive to semantic structure in addition to the surface syntax. (Bock and Loebell (1990) also addressed the question of whether thematic roles contribute to priming, seemingly finding evidence that they do not.) - \textit{Event Structures Drive Semantic Structural Priming, Not Thematic Roles: Evidence From Idioms and Light Verbs}


\subsection{Semantic role}
In the dative construction, the semantic roles are agent (subject), recipient (object) and theme (indirect object).


Unigram probability of all tokens given chosen model
average perplexity of sentences with no prime per structure
E.g. comparing between can tell us about model pref for one struct vs other? Some baseline from which to interpret model size and also relative act pass differences
One also for animate vs inanimate roles
recency of lext boost effects
Relative effect of sem sim on structure
Explore effect of given a certain point in the sentence: possible scope of structure narrows
The woman threw the stick to the dog → The boy gave the book to the man
The woman threw the dog the stick →The boy gave the man the book
Include only semsim, lexboost and semantically related modifier condition from complex NP in analysis? 
Will implausible primes give us anything useful wrt question? → maybe yes to confirm this semantic role idea (e.g. it is not fulfilled → lower priming?) but could be confusing since model should be v perplexed by them in general



\subsection{Research Questions}
\begin{itemize}
    \item Model scale shows increased performance on tasks, but does this mean they retain higher level abstract psycholinguistic properties (e.g. estimates from GPT-2~\citep{Radford2019LanguageMA} have been shown to be predictive of comprehension behaviour, even more so than larger LM variants \citep{shain2022large,oh2023does})
    \item How do alignment optimisation procedures such as RLHF and DPO---shown to improve human perception of model output---affect how human like their comprehension behaviour is? 
    \item Do linguistic factors play an important role in influencing model predictions over the target, if so are these reflective of results found in linguistic corpus studies?
    \item 
\end{itemize}

\paragraph{Related + Motivation}

\begin{itemize}
    \item Many factors influence priming behaviour in humans. Isolating for lexical overlap in humans has found to remove priming effects completely in some studies. priming can be influenced by  factors such as semantic role, common lexical pairings, preferences for certain lexical items in certain structures (e.g. verb x for DO) in humans. 
    \item 
    \item \cite{arehalli2022syntactic} Syntactic surprisal from neural models predicts, but underestimates, human processing difficulty from syntactic ambiguities. Models underestimate garden paths because humans are more concerned with interpretation, whereas models are not hierarchically doing much. 
    % \item Investigating the extent to which Neural Language Models (NLMs) successfully encode structure has the potential to help answer long standing debates within theoretical linguistics e.g.~\cite{linzen2021syntactic}
    \item Priming effects can also be explained at the level of constructions (in contrast to lexicalist linguistic theories which assume argument structure is predictable from the meaning of the verb only), construction grammar posits constructions (or form-meaning pairs) encode argument structure. 
    %$\rightarrow$ \textit{e.g. we may want to explore the constructions as well as the individual tokens. e.g. 'to the man' 'from the boy'} 
    \cite{li2022neural} test this using a “Jabberwocky” priming-based experiment, highlighting that models associate meaning with constructions even in semantically nonsensical sentences. \cite{sinclair2022structural} find biased priming effects with similarly ``implausible'' priming sentences, we therefore inspect whether exploring priming effects at a more fine-grained construction or token level allows for further insights about where these biased effects occur. 
    % \textit{``Second, in a “Jabberwocky” priming-based experiment, we find that LMs associate ASCs with meaning, even in semantically nonsensical sentences. Our work offers the first evidence for ASCs in LMs and highlights the potential to devise novel probing methods grounded in psycholinguistic research.''} 
    $\rightarrow$ constructions and these sorts of constraints.  
    % (\textit{``In lexicalist linguistic theories, argument structure is assumed to be predictable from the meaning of verbs. As a result, the verb is the primary determinant of the meaning of a clause. In contrast, construction grammarians propose that argument structure is encoded in constructions (or form-meaning pairs) that are distinct from verbs. Decades of psycholinguistic research have produced substantial empirical evidence in favor of the construction view.''} )
    \item \cite{trueswell1993verb} \textit{Verb-specific constraints in sentence processing: separating effects of lexical preference from garden-paths.} $\rightarrow$ fits in with verb analysis: verb pref for certain structures. 
    \item DO easier and preferred, PO harder, less preferred. 
    \item \cite{shain2020fmri} \textit{fMRI reveals language-specific predictive coding during naturalistic sentence comprehension}
    \item What do we mean by prediction in language comprehension? \cite{kuperberg2016we} 
    \item  Probing for Incremental Parse States in Autoregressive Language Models. \cite{eisape2022probing} suggest that implicit incremental syntactic inferences underlie next-word predictions in autoregressive neural language models. We inspect token level priming effects to explore the onset of the priming behaviour within the sentence, to understand at what point the presence of the congruent structure influences model predictions over the structure of the target.
    \item \cite{wilcox2021targeted} perform targeted assessment of incremental processing in Humans and NLMs, and highlight the importance for evaluating local fluctuations in processing difficulty (as measured by surprisal): e.g. certain local areas may contain higher levels of syntactic ambiguity, these effects would be hidden by sentence level.  
    \item \cite{shen2020explicitly} point out that although some NLMs excel at having low perplexity scores, this is less due to their syntactic ability but more due to capturing collocations (frequently co-occurring words), we thus investigate the extent to which these effects may influence our priming effects. 
    \item 
\end{itemize}



\paragraph{Experiments} 
\begin{enumerate}
    \item We first inspect a suite of contemporary pretrained \textit{Transformer} language models for their susceptibility to priming, and the extent to which lexical vs structural relationships between primes and targets affects the relative boost in PE. (graph of biased vs unbiased effects and movement)
    \item We then investigate 
\end{enumerate}

%Explicitly Modeling Syntax in Language Models with Incremental Parsing and a Dynamic Oracle
%Several recent works have systematically studied
% the linguistic abilities of modern language models,
% particularly syntax (Linzen et al., 2016; Marvin and
% Linzen, 2018; Gulordava et al., 2018). They find
% that most language models are good at capturing
% frequent syntactic structures but do not generalize
% well to those in the long tail. Moreover, although
% some excel at having low perplexity scores, this
% is less due to their syntactic ability but more due
% to capturing collocations (frequently co-occurring
% words). Recently, Hu et al. (2020) show that RNNs
% underperform on a syntactic generalization (SG)
% test set, whereas models that have an explicit notion
% of syntax, such as RNNG (Dyer et al., 2016), fare
% well on SG but at the cost of generally poorer language modeling (higher perplexity). Transformerbased models achieve strong performance when
% trained with large datasets, but are worse than random when trained on a small dataset.


%A Targeted Assessment of Incremental Processing in Neural Language Models and Humans
%Multiple options exist that could magnify surprisal values in
% locally ambiguous or ungrammatical regions, such
% as a reduced beam size (Roark, 2001) or particle
% filters (Levy et al., 2009). Taken together, these
% recent results highlight a key question for future
% research—what additional modeling mechanisms
% will be needed to accurately predict not only qualitative but also quantitative patterns of human difficulty in language processing.

%Probing for Incremental Parse States in Autoregressive Language Models
% Next-word predictions from autoregressive
% neural language models show remarkable sensitivity to syntax. This work evaluates the extent to which this behavior arises as a result
% of a learned ability to maintain implicit representations of incremental syntactic structures.
% We extend work in syntactic probing to the incremental setting and present several probes
% for extracting incomplete syntactic structure
% (operationalized through parse states from a
% stack-based parser) from autoregressive language models. We find that our probes can
% be used to predict model preferences on ambiguous sentence prefixes and causally intervene on model representations and steer model
% behavior. This suggests implicit incremental
% syntactic inferences underlie next-word predictions in autoregressive neural language models


